A mechanics theory for the exploration of a high-throughput, sterile 3D $\textit{in vitro}$ traumatic brain injury model

Brain injuries resulting from mechanical trauma represent an ongoing global public health issue. Several $\textit{in vitro}$ and $\textit{in vivo}$ models for traumatic brain injury (TBI) continue to be developed for delineating the various complex pathophysiological processes involved in its onset and progression. Developing an $\textit{in vitro}$ TBI model that is based on cortical spheroids is especially of great interest currently because they can replicate key aspects of $\textit{in vivo}$ brain tissue, including its electrophysiology, physicochemical microenvironment, and extracellular matrix composition. Being able to mechanically deform the spheroids is a key requirement in any effective $\textit{in vitro}$ TBI model. The spheroids' shape and size, however, make mechanically loading them, especially in a high-throughput, sterile, and reproducible manner, quite challenging. To address this challenge, we present an idea for a spheroid-based, $\textit{in vitro}$ TBI model in which the spheroids are mechanically loaded by being spun by a centrifuge. (An experimental demonstration of this new idea will be published shortly elsewhere.) An issue that can limit its utility and scope is that imaging techniques used in 2D and 3D $\textit{in vitro}$ TBI models cannot be readily applied in it to determine spheroid strains. In order to address this issue, we developed a continuum mechanics-based theory to estimate the spheroids' strains when they are being spun at a constant angular velocity. The mechanics theory, while applicable here to a special case of the centrifuge-based TBI model, is also of general value since it can help with the further exploration and development of TBI models.

==> fonttable.tex <==
\begin{equation}
\begin{array}{rll}
 \verb !W_{ij} Q_{im} \gamma! &   W_{ij}Q_{im} \gamma \\
    \verb!\boldsymbol{\gamma}!& \boldsymbol{\gamma}\\
    \verb!\sgamma! & \sgamma \\ 
    \verb!\sfgamma! & \sfgamma \\
    \verb!\bsfgamma! & \bsfgamma\\
    \verb!g! & g\\
    \verb!\boldsymbol{g}! &\boldsymbol{g} \\
    \verb!\mathbf{g}! &     \mathbf{g}\\ 
    \verb!\mathsf{g}!&\mathsf{g}\\
    \verb!\mathit{g}! &     \mathit{g}\\ 
    \verb!\mathit{\mathsf{g}}!&\mathit{\mathsf{g}}\\
    \verb!\mathsf{\mathit{g}}!&\mathsf{\mathit{g}}\\
    \verb!\boldsymbol{\mathit{g}}!&\boldsymbol{\mathit{g}}\\
    \verb!G! & G & *\\
    \verb!\mathsf{G}!&\mathsf{G} & * \\
    \verb!\boldsymbol{\mathsf{G}}!&\boldsymbol{\mathsf{G}} & *\\
    \verb!\sG!& \sG & *\\
    \verb!\sfmitG!& \sfmitG & * \\
    \verb!\sfbitG! & \sfbitG & * \\
    \verb!\mathbf{G}! &     \mathbf{G} & *\\ 
    \verb!\mathcal{G}! & \mathcal{G} & * \\
    \verb!\calG! &     \calG & *\\ 
    \verb!\boldsymbol{G}! &\boldsymbol{G} \\
    
    
    \verb!\mathit{G}! &     \mathit{G}\\ 
    \verb!\mathit{\mathsf{G}}!&\mathit{\mathsf{G}}\\
    \verb!\mathsf{\mathit{G}}!&\mathsf{\mathit{G}}\\
    
    \verb!\boldsymbol{\mathit{G}}!&\boldsymbol{\mathit{G}}\\    
    \verb!\sfmnG! & \sfmnG &  \\
    \verb!\mathbf{\sG}! & \mathbf{\sG}\\
    \verb!\calA! &\calA\\
\end{array}
\end{equation}

==> notes.tex <==
The left and right Cauchy-Green deformation tensor corresponding to the deformation gradient $F_{ij}\ag{\usf{X}}\bl{e}_i\ag{\tau}\otimes \bl{E}_j$ are, respectively,
\begin{subequations}
\begin{equation}
\bl{B}_{\bl{\tau}}\ag{\bl{X}}=B_{ij}\ag{\usf{X}}\bl{e}_i\ag{\tau}\otimes \bl{e}_j\ag{\tau},
\end{equation}
where
\begin{equation}
B_{ij}\ag{\usf{X}}=F_{im}\ag{\usf{X}}F_{jm}\ag{\usf{X}},
\end{equation}
\label{eq:leftcauchygreen}
\end{subequations}
and 
\begin{subequations}
\begin{equation}
\bl{C}\ag{\bl{X}}=C_{ij}\ag{\usf{X}}\bl{E}_{i}\otimes \bl{E}_j,
\end{equation}
where
\begin{equation}
C_{ij}\ag{\usf{X}}=F_{mi}\ag{\usf{X}}F_{mj}\ag{\usf{X}}.
\end{equation}
\end{subequations}
We abbreviate $\pr{F_{ij}\ag{\usf{X}}}_{i,j\in \mathcal{I}}$, $\pr{B_{ij}\ag{\usf{X}}}_{i,j\in \mathcal{I}}$, and $\pr{C_{ij}\ag{\usf{X}}}_{i,j\in \mathcal{I}}$ as $\usf{F}\ag{\usf{X}}$, $\usf{B}\ag{\usf{X}}$, and $\usf{C}\ag{\usf{X}}$, respectively.
